A Survey on Deep Learning and Explainability for Automatic Report Generation from Medical Images

Every year physicians face an increasing demand of image-based diagnosis from patients, a problem that can be addressed with recent artificial intelligence methods. In this context, we survey works in the area of automatic report generation from medical images, with emphasis on methods using deep neural networks, with respect to: (1) Datasets, (2) Architecture Design, (3) Explainability and (4) Evaluation Metrics. Our survey identifies interesting developments, but also remaining challenges. Among them, the current evaluation of generated reports is especially weak, since it mostly relies on traditional Natural Language Processing (NLP) metrics, which do not accurately capture medical correctness.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> custom-comments.tex <==
\newcommand{\ppino}[1]{\textcolor{blue}{\textbf{Pablo Pino}: #1}}
\newcommand{\pamessina}[1]{\textcolor{green}{\textbf{Pablo Messina}: #1}}

\newcommand{\customComment}[3]{{\colorbox{#2}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
{\textcolor{#2}{\sf\small\textit{#3}}}}

\newcommand{\todo}[1]{\customComment{TODO}{red}{#1}}
%% Usar \todo{TODO comment}, para cualquier TODO que lo puede completar cualquiera.

\newcommand{\review}[1]{\customComment{REVIEW}{orange}{#1}}
%% Usar \review{TEXTO} para algo que haya que revisar

\newcommand{\citemissing}[1]{\customComment{CITE}{violet}{#1}}
%% Usar \citemissing{TEXTO} para indicar que falta una cita. El texto es opcional


% \usepackage{refcheck}
% INCLUDE IN DOCUMENT BODY TO CHECK UNUSED CITES:
% \nocite{*}



% \usepackage{xcolor}
% \definecolor{red-strong}{RGB}{231, 19, 19}
% \definecolor{red-light}{RGB}{223, 78, 78}

% \definecolor{red-strong}{RGB}{246, 101, 4}
% \definecolor{red-light}{RGB}{252, 155, 89}

==> tables/datasets-extra-data-public-only.tex <==
\newcommand{\datasetCellEmpty}{\multicolumn{1}{c|}{-}}
% \newcommand{\datasetCXRBB}{$^{\textrm{(1)}}$}

\def\addedColSepDatasets{1pt}
% \def\flushboth{%
%   \let\\\@normalcr
%   \@rightskip\z@skip \rightskip\@rightskip
%   \leftskip\z@skip
%   \parindent 1.5em\relax}

\addtolength{\tabcolsep}{-\addedColSepDatasets{}}


\begin{table}[htbp]
% \small
\scalebox{0.8}{
\begin{tabular}{|p{0.25\linewidth}|p{0.1\linewidth}|p{0.32\linewidth}|p{0.22\linewidth}|p{0.25\linewidth}|}
\hline
\textbf{Dataset} & \textbf{Text} & \textbf{Tags} & \raggedright{\textbf{Tags annotation method}} & \textbf{Localization} \\ \hline
\multicolumn{5}{|c|}{\textbf{Public report datasets}} \\ \hline
IU X-ray \cite{10.1093/jamia/ocv080} & Indication & (1) MeSH and RadLex concepts (2) MeSH concepts & \raggedright{(1) Manual (2) MTI and MetaMap} & \datasetCellEmpty \tabularnewline \hline
MIMIC-CXR \cite{johnson2019mimicv1, johnson2019mimiccxrjpg} & \datasetCellEmpty & 14 CheXpert labels & CheXpert labeler and NegBio & \datasetCellEmpty \tabularnewline \hline
PadChest \cite{bustos2019padchest} & \datasetCellEmpty & 297 labels (findings, diagnoses and anatomic) & \raggedright{27\% manual, rest by RNN} & \datasetCellEmpty \tabularnewline \hline
\raggedright{ImageCLEF Caption 2017 \cite{eickhoff2017overview}} & \datasetCellEmpty & UMLS tags & Quick-UMLS & \datasetCellEmpty \\ \hline
\raggedright{ImageCLEF Caption 2018 \cite{de2018overview}} & \datasetCellEmpty & UMLS tags & Quick-UMLS & \datasetCellEmpty \\ \hline
ROCO \cite{dataset2018roco} & \datasetCellEmpty & UMLS tags & Quick-UMLS & \datasetCellEmpty \\ \hline
PEIR Gross \cite{jing2017automatic} & \datasetCellEmpty & Top words & Top TF-IDF scores & \datasetCellEmpty \\ \hline
INBreast \cite{moreira2012inbreast} & \datasetCellEmpty & Abnormalities & Manual & \raggedright{Abnormality contours} \tabularnewline \hline
STARE \cite{hoover1975stare} & \datasetCellEmpty & \raggedright{Levels for 39 conditions and presence of 13 diagnostics} & Manual & \datasetCellEmpty \\ \hline
RDIF \cite{maksoud2019coral8} & Indication & \datasetCellEmpty & \datasetCellEmpty & \datasetCellEmpty \\ \hline\hline
\multicolumn{5}{|c|}{\textbf{Public classification datasets}} \\ \hline
CheXpert \cite{irvin2019chexpert} & \datasetCellEmpty & 14 CheXpert labels & CheXpert labeler & \datasetCellEmpty \\ \hline
ChestX-ray14 \cite{Wang_2017_CVPR} & \datasetCellEmpty & 14 disease labels & DNorm and MetaMap & \raggedright{Disease bounding boxes for 880 images} \tabularnewline \hline
LiTS \cite{christ2017lits} & \datasetCellEmpty & \datasetCellEmpty & \datasetCellEmpty & \raggedright{Liver and tumor segmentation masks} \tabularnewline \hline
\raggedright{Gastrointestinal challenge \cite{10.1145/3343031.3356058}} & \datasetCellEmpty & 16 labels (e.g. anatomic, pathological or surgery findings) & Manual & \datasetCellEmpty \\ \hline
DIARETDB0 \cite{kauppi2006diaretdb0} & \datasetCellEmpty & DR severity level & Manual & Abnormality contours \\ \hline
DIARETDB1 \cite{kalviainen2007diaretdb1} & \datasetCellEmpty & DR severity level & Manual & Abnormality contours \\ \hline
Messidor \cite{decenciere2014feedback, abramoff2013automated} & \datasetCellEmpty & DR severity level & Manual & \datasetCellEmpty \\ \hline
DDSM \cite{heath2001digital} & \datasetCellEmpty & Density level & Manual & \raggedright{Abnormalities at pixel level} \tabularnewline \hline
\end{tabular}
}
\caption{Additional data contained in each dataset.
    MeSH \cite{rogers1963medical} and RadLex \cite{langlotz2006radlex} are sets of medical concepts.
    MTI \cite{mork2013nlm}, MetaMap \cite{aronson2010overview}, CheXpert labeler \cite{irvin2019chexpert}, NegBio \cite{peng2018negbio}, Quick-UMLS \cite{soldaini2016quickumls} and DNorm \cite{leaman2015challenges} are automatic labeler tools.
    \textit{Manual} means manually annotated by experts.
    % \datasetCXRBB: bounding boxes are only available for 880 images.
    In all cases, the localization information was manually annotated by experts.
    }
\label{table:datasets-extra-data}
\end{table}

\addtolength{\tabcolsep}{\addedColSepDatasets{}}

==> tables/domain-knowledge.tex <==
\begin{table}[ht]
% \begin{tabular}{|p{0.36\textwidth}|p{0.16\textwidth}|}
\scalebox{0.8}{
\begin{tabular}{|l|l|}
\hline
 \textbf{Category}  & \textbf{Used by papers}
 \\ \hline
 Knowledge-based graph neural network &
 \cite{li2019knowledge, zhang2020radiology}\\
 
 Template database &
 \cite{li2018hybrid, li2019knowledge, biswal2020clara, 10.1145/3343031.3356066, 10.1007/978-3-030-00937-3_22, kisilev2016medical, moradi2016cross}\\
 \hline
\end{tabular}
}
\caption{Summary of domain knowledge practices identified in the literature.}
\label{tab:dk}
\end{table}


==> tables/iu-xray-results.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{images/results-papers-Open-I.png}
% \end{figure}

\newcommand{\tableSotaComment}[1]{$^{\textrm{(#1)}}$}

\def\addedColSep{2.5pt}

\addtolength{\tabcolsep}{-\addedColSep{}}

\begin{table}[tbp]
% \small
\scalebox{0.8}{
\begin{tabular}{|l|cccc|c|c|cc|}
\hline
\textbf{Paper} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{ROUGE-L} & \textbf{METEOR} & \textbf{CIDEr} & \textbf{CIDEr-D} \\ \hline
\multicolumn{9}{|c|}{\textbf{Findings section}} \\ \hline
Liu et al. \cite{liu2019clinically} & 0.369 & 0.246 & 0.171 & 0.115 & 0.359 & - & \textbf{-} & \textbf{1.490} \\
HRGR \cite{li2018hybrid} & 0.438 & 0.298 & 0.208 & 0.151 & 0.369 & - & - & 0.343 \\
KERP \cite{li2019knowledge} & \textbf{0.482} & \textbf{0.325} & \textbf{0.226} & 0.162 & 0.339 & - & - & 0.280 \\
TieNet \cite{wang2018tienet} \tableSotaComment{1} & 0.330 & 0.194 & 0.124 & 0.081 & 0.311 & - & - & 1.334 \\
Xue et al. 2018 \cite{xue2018multimodal} \tableSotaComment{2} & 0.441 & 0.320 & 0.231 & 0.181 & 0.366 & 0.220 & 0.343 & - \\
RTMIC \cite{xiong2019reinforced} & 0.350 & 0.234 & 0.143 & 0.096 & - & - & 0.323 & - \\
CLARA \cite{biswal2020clara} \tableSotaComment{3} & 0.471 & 0.324 & 0.214 & \textbf{0.199} & - & - & \textbf{0.359} & - \\
Xue et al. 2019 \cite{10.1007/978-3-030-20351-1_10} & 0.477 & 0.332 & 0.243 & 0.189 & \textbf{0.380} & \textbf{0.223} & 0.320 & - \\
CMAS \cite{jing2019show} & 0.464 & 0.301 & 0.210 & 0.154 & 0.362 & - & - & 0.275 \\ \hline
\multicolumn{9}{|c|}{\textbf{Findings section - Cardiomegaly sentences only}} \\ \hline
Spinks and Moens \cite{spinks2019justifying} & 0.490 & 0.350 & 0.250 & 0.180 & 0.400 & 0.270 & 0.600 & - \\
\hline
\multicolumn{9}{|c|}{\textbf{Impression section}} \\ \hline
MTMA \cite{10.1007/978-3-030-33850-3_8} & \textbf{0.882} & \textbf{0.874} & \textbf{0.867} & \textbf{0.860} & \textbf{0.929} & - & - & - \\
CMAS \cite{jing2019show} & 0.401 & 0.290 & 0.220 & 0.166 & 0.521 & - & - & 1.457 \\ \hline
\multicolumn{9}{|c|}{\textbf{Findings + Impression sections}} \\ \hline
CoAtt \cite{jing2017automatic} & 0.517 & \textbf{0.386} & 0.306 & 0.247 & 0.447 & 0.217 & - & 0.327 \\
Huang et al. \cite{huang2019multi} & 0.476 & 0.340 & 0.238 & 0.169 & 0.347 & - & 0.297 & - \\
Yuan et al. \cite{yuan2019automatic} & \textbf{0.529} & 0.372 & 0.315 & 0.255 & 0.453 & \textbf{0.343} & - & - \\
Xue et al. 2018 \cite{xue2018multimodal} & 0.464 & 0.358 & 0.270 & 0.195 & 0.366 & 0.274 & - & - \\
Vispi \cite{li2019vispi} & 0.419 & 0.280 & 0.201 & 0.150 & 0.371 & - & 0.553 & - \\
Singh et al. \cite{singh2019chest} & 0.374 & 0.224 & 0.153 & 0.110 & 0.308 & 0.164 & 0.360 & - \\
Yin et al. \cite{8970668} & 0.445 & 0.292 & 0.201 & 0.154 & 0.344 & 0.175 & 0.342 & - \\
MLMA \cite{10.1007/978-981-15-4015-8_15} & 0.500 & 0.380 & \textbf{0.317} & \textbf{0.278} & 0.440 & 0.281 & - & \textbf{1.067} \\
Harzig et al. 2019a \cite{harzig2019addressing} & 0.373 & 0.246 & 0.175 & 0.126 & 0.315 & 0.163 & 0.359 & - \\
A3FN \cite{10.1007/978-3-030-18590-9_64} & 0.443 & 0.337 & 0.236 & 0.181 & 0.347 & - & 0.374 & - \\
Xue et al. 2019 \cite{10.1007/978-3-030-20351-1_10} & 0.489 & 0.340 & 0.252 & 0.195 & \textbf{0.478} & 0.230 & \textbf{0.565} &  \\
Zhang et al. \cite{zhang2020radiology} & 0.441 & 0.291 & 0.203 & 0.147 & 0.367 & - & 0.304 & - \\ \hline
\end{tabular}
}
\caption{Evaluation results of papers that use the IU X-ray dataset.
    All values were extracted from their papers, except in some cases where results were not present in the own paper:
    \tableSotaComment{1} TieNet \cite{wang2018tienet} results were presented in Liu et al. \cite{liu2019clinically} as a baseline;
    \tableSotaComment{2} Xue et al. 2018 \cite{xue2018multimodal} results in the findings section were presented in Xue et al. 2019 \cite{10.1007/978-3-030-20351-1_10} as a baseline.
    \tableSotaComment{3} CLARA \cite{biswal2020clara} results are from the fully automatic version.
    }
\label{table:iu-xray-results}
\vspace{-8mm}
\end{table}
%\vspace{-3mm}

\addtolength{\tabcolsep}{\addedColSep{}}

==> tables/models-by-paper.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/Table-Models.png}
    \caption{Summary of model architectures in the literature. Best viewed in PDF with zoom.
    (*) ad-hoc architecure.
    LIRE (\^{}) is a library for extracting traditional visual features such as color histograms, texture features, etc (non-DL).
    Lucene (\^{} *) is a software package for text-based information retrieval.
    (\^{}\^{}) These models re-read what they have generated so far to predict the next word (complexity $O(N^2)$, where $N$ is the length of the final report).
    CLARA (\&) has two versions: \textit{human-in-the-loop}, and \textit{automatic}; when unspecified, the entry is valid for both versions.
    Hierarchical LSTM refers to one LSTM for sentences, and one for words.
    LSTM alone generates a full report word by word.
    \textit{indication} is a free text indicated by the physician requesting the imaging exam, while \textit{findings} is the section of the report describing findings in the image.
    \textit{template database} is a set of template sentences, arranged in a specific way.
    MLC stands for Multi-Label Classification, FCN stands for Fully Convolutional Network, and FC stands for Fully Connected.
    }
    \label{table:models-by-paper}
\end{figure}

==> tables/optimization-by-paper.tex <==
\newcommand{\optTableVispi}{$^{\textrm{(1)}}$}
\newcommand{\optTableGAN}{$^{\textrm{(2)}}$}
\newcommand{\optTableNotSure}{?}
\newcommand{\rotatedHeader}[1]{\rotatebox[origin=c]{90}{\textbf{#1}}}


\begin{table}[htpb]
% \small
\scalebox{0.8}{
\begin{tabular}{|p{0.25\linewidth}|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Paper}}} & \multicolumn{3}{c|}{\textbf{Visual Component}} & \multicolumn{2}{c|}{\textbf{Report Generation}} & \multicolumn{4}{c|}{\textbf{Other Tasks or Losses}} \\ \cline{2-10} 
\multicolumn{1}{|c|}{} & \rotatedHeader{ImageNet} & \rotatedHeader{Medical Image Tasks} & \rotatedHeader{Report Generation} & \rotatedHeader{Teacher Forcing} & \rotatedHeader{RL} & \rotatedHeader{Att. weights Reg.} & \rotatedHeader{Contrastive Loss} & \rotatedHeader{GAN} & \rotatedHeader{Autoencoder} \\ \hline
CoAtt \cite{jing2017automatic} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & X & \multicolumn{1}{c|}{X} &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
Liu et al. \cite{liu2019clinically} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & X &  & \multicolumn{1}{c|}{X} &  &  &  &  \\ \hline
Huang et al. \cite{huang2019multi} & X &  & \optTableNotSure & X &  &  &  &  &  \\ \hline
Yuan et al. \cite{yuan2019automatic} & \multicolumn{1}{l|}{} & X &  & X &  &  &  &  &  \\ \hline
HRGR \cite{li2018hybrid} & X & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{c|}{X} &  &  &  &  \\ \hline
KERP \cite{li2019knowledge} & \multicolumn{1}{l|}{} & X &  & X &  &  &  &  &  \\ \hline
TieNet \cite{wang2018tienet} & X & \multicolumn{1}{l|}{} & X & X &  &  &  &  &  \\ \hline
Xue et al. 2018 \cite{xue2018multimodal} & X & \multicolumn{1}{l|}{} &  & X &  &  &  &  &  \\ \hline
MDNet \cite{zhang2017mdnet} & \multicolumn{1}{l|}{} & X & X & X &  &  &  &  &  \\ \hline
Vispi \optTableVispi \cite{li2019vispi} & X & X &  & X &  &  &  &  &  \\ \hline
RTMIC \cite{xiong2019reinforced} & \multicolumn{1}{l|}{} & X &  &  & \multicolumn{1}{c|}{X} &  &  &  &  \\ \hline
Singh et al. \cite{singh2019chest} & X & \multicolumn{1}{l|}{} &  & X &  &  &  &  &  \\ \hline
CORAL8 \cite{maksoud2019coral8} & X & \multicolumn{1}{l|}{} &  & X &  & X &  &  &  \\ \hline
Gale et al. \cite{gale2018producing} &  & X &  & \multicolumn{1}{c|}{X} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
Tian et al. \cite{10.1007/978-3-030-00934-2_78} &  & X & X & X &  &  &  &  &  \\ \hline
Gu et al. \cite{8935910} &  & X &  & X &  &  &  &  &  \\ \hline
Yin et al. \cite{8970668} & X & X & X & X &  & X & X &  &  \\ \hline
MTMA \cite{10.1007/978-3-030-33850-3_8} &  & X & \optTableNotSure & X &  &  &  &  & X \\ \hline
Ma et al. \cite{10.1007/978-3-030-04224-0_24} & X & X &  &  &  &  &  &  &  \\ \hline
Alsharid et al. \cite{10.1007/978-3-030-32251-9_37} & X & X & \optTableNotSure & X &  & \multicolumn{1}{l|}{} &  &  &  \\ \hline
Gasimova et al. \cite{gasimova2019automated} & X &  & X & X &  &  &  &  &  \\ \hline
MLMA \cite{10.1007/978-981-15-4015-8_15} & \optTableNotSure &  & \optTableNotSure & X &  &  &  &  &  \\ \hline
Harzig et al. 2019a \cite{harzig2019addressing} &  & X & X & X &  &  &  &  &  \\ \hline
CLARA \cite{biswal2020clara} & \optTableNotSure & X & \optTableNotSure & X &  &  &  &  &  \\ \hline
A3FN \cite{10.1007/978-3-030-18590-9_64} & \optTableNotSure &  & \optTableNotSure & X &  &  &  &  &  \\ \hline
Zeng et al. \cite{Zeng2018} & X & X &  & X &  &  &  &  &  \\ \hline
Harzig et al. 2019b \cite{10.1145/3343031.3356066} &  & X &  &  &  &  &  &  &  \\ \hline
Xue et al. 2019 \cite{10.1007/978-3-030-20351-1_10} & X &  & X & X &  &  &  &  &  \\ \hline
Sun et al. \cite{10.1007/978-3-030-26763-6_66} &  & X &  & X &  &  &  &  &  \\ \hline
Zhang et al. \cite{zhang2020radiology} &  & X &  & X &  &  &  &  &  \\ \hline
Han et al. \cite{10.1007/978-3-030-00937-3_22} &  & X\optTableGAN &  &  &  &  &  & X &  \\ \hline
Li et al. \cite{10.1145/3357254.3357256} &  &  & X\optTableGAN & X & \multicolumn{1}{c|}{X\optTableGAN} &  &  & X &  \\ \hline
CMAS \cite{jing2019show} & X & X &  & X & \multicolumn{1}{c|}{X} &  &  &  &  \\ \hline
Shin et al. \cite{Shin_2016_CVPR} & \optTableNotSure & X &  & X &  &  &  &  &  \\ \hline
Hasan et al. \cite{10.1007/978-3-319-98932-7_21} & X & X & X & X &  &  &  &  &  \\ \hline
% Mishra et al. \cite{Mishra2020} & X &  &  & X &  &  &  &  &  \\ \hline
% Zhang and Wang et al. \cite{zhang2018imagesem} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
}
\caption{Summary of optimization strategies per paper. \optTableVispi In Vispi, ResNet 101 is pre-trained in ImageNet, and DenseNet 121 is trained in auxiliary medical image task. Marks with \optTableGAN are trained using a GAN architecture.
Boxes marked with \optTableNotSure{} mean it was not clear from the paper manuscript.
}
\label{table:optimization-by-paper}
\end{table}
